Electron-Muon Ranger: hardware characterization

The Electron-Muon Ranger (EMR) is a fully-active tracking-calorimeter in charge of the electron background rejection downstream of the cooling channel at the international Muon Ionization Cooling Experiment. It consists of 2832 plastic scintillator bars segmented in 48 planes in an X-Y arrangement and uses particle range as its main variable to tag muons and discriminate electrons. An array of analyses were conducted to characterize the hardware of the EMR and determine whether the detector performs to specifications. The clear fibres coming from the bars were shown to transmit the desired amount of light, and only four dead channels were identified in the electronics. Two channels had indubitably been mismatched during assembly and the DAQ channel map was subsequently corrected. The level of crosstalk is within acceptable values for the type of multi-anode photomultiplier used with an average of $0.20\pm0.03\,\%$ probability of occurrence in adjacent channels and a mean amplitude equivalent to $4.5\pm0.1\,\%$ of the primary signal intensity. The efficiency of the signal acquisition, defined as the probability of recording a signal in a plane when a particle goes through it in beam conditions, reached $99.73\pm0.02\,\%$.

==> GetPackages.tex <==
\usepackage{lineno}
\usepackage{bibentry}
\nobibliography*
\usepackage{times}
\usepackage{bm}         % bold maths
\usepackage{amsmath,amssymb,bm,slashed} % need for subequations
\usepackage{amssymb}    % extra math symbols
\usepackage{graphicx}   % need for figures
\usepackage{verbatim}   % useful for program listings
\usepackage{color}      % use if color is used in text
\usepackage{subfigure}  % use for side-by-side figures
\usepackage{hyperref}   % use for hypertext links, including those to external documents and URLs
\usepackage{enumerate}
\usepackage{lineno}
\usepackage{textcomp}

\usepackage{fmtcount}   % Allow counters to be printed with padding

\usepackage[square,comma,numbers,sort&compress]{natbib}


